Efficient periodic density functional theory calculations of charged molecules and surfaces using Coulomb kernel truncation

Density functional theory (DFT) calculations of charged molecules and surfaces are critical to applications in electro-catalysis, energy materials and related fields of materials science. DFT implementations such as the Vienna ab-initio Simulation Package (VASP) compute the electrostatic potential under 3D periodic boundary conditions, necessitating charge neutrality. In this work, we implement 0D and 2D periodic boundary conditions to facilitate DFT calculations of charged molecules and surfaces respectively. We implement these boundary conditions using the Coulomb kernel truncation method. Our implementation computes the potential under 0D and 2D boundary conditions by selectively subtracting unwanted long-range interactions in the potential computed under 3D boundary conditions. By combining the Coulomb kernel truncation method with a computationally efficient padding approach, we remove nonphysical potentials from vacuum in 0D and 2D systems. To illustrate the computational efficiency of our method, we perform large supercell calculations of the formation energy of a charged chlorine defect on a sodium chloride (001) surface and perform long time-scale molecular dynamics simulations on a stepped gold (211) | water electrode-electrolyte interface.

==> charged_adsorbate.tex <==
\subsection{Adsorbate on a metallic surface}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figures/charged_adsorbate.png}
    \caption{a) Energy referenced to the energy at zero charge as a function of the number of added electrons for (blue) 3D periodic calculations (green) 2D periodic calculations of carbon adsorbed on the top site of an Al(111) surface b) Fermi energy referenced to the fermi energy at no added charge as a function of the number of added electrons.}
    \label{fig:charged-adsorbate}
\end{figure}


